Ontology Engineering to Model the European Cultural Heritage: The Case of Cultural Gems

Cultural gems is a web application conceived by the European Commission's Joint Research Centre (DG JRC), which aims at engaging people and organisations across Europe to create a unique repository of cultural and creative places. The main goal is to provide a vision of European culture in order to strengthen a sense of identity within a single European cultural realm. Cultural gems maps more than 130,000 physical places in over 300 European cities and towns, and since 2020 it also lists online cultural initiatives. The new release aims, among other, to increase the interoperability of the application. At this purpose, we provide an overview on the current development of an ontology for Cultural gems used to map cultural heritage in European cities by using Linked Open Data (LOD) standards, and making the data FAIR, that is Findable, Accessible, Interoperable, and Reusable. We provide an overview of the methodology, presenting the structure of the ontology, and the services and tools we are currently building on top.

==> navigator.tex <==
% This is the Navigator package.
% Relevant information can be found in navigator-doc.pdf
%
% Author: Paul Isambert.
% E-mail: zappathustra AT free DOT fr
% Comments and suggestions are welcome.
% Date: January 2011.

\ifdefined\NavigatorHasAlreadyBeenLoadedMyDear
  \expandafter\endinput
\fi
\let\NavigatorHasAlreadyBeenLoadedMyDear\relax

\input yax
\ifdim\yaxversion pt<1.03pt
  \senderror{Navigator}{YaX should be at least version 1.03. I quit}%
  \expandafter\endinput
\fi

\ifnum\texenginenumber>1
  \lettocs\ifpdforluatex{iftrue}
\else
  \letcstocs{ifpdforluatex}{iffalse}
\fi
\newsyntax#1:#2;{nav@}
\setcatcodes{_@=11}
\def\nav@error#1{\senderror{Navigator}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% Strings %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifcase\texenginenumber
\or
% XeTeX: we do nothing. Under some circumstances,
% xdvipdfmx writes a good UTF-16 string.
\let\pdfstring\unbrace

\or
% PDFTeX: we escape the string.
\let\pdfstring\pdfescapestring

\or
% LuaTeX: the string is converted from UTF-8 to
% UTF-16, and expressed in octal form (otherwise LuaTeX
% would complain about non-UTF-8 characters). Hexadecimal
% strings may be better, but \pdfoutline encloses the title
% between braces, whereas hexadecimal strings should be
% enclosed between "<" and ">".
%
% The UTF-16 conversion covers the entire Unicode range,
% because one has the right to use Linear-B or musical notations
% in a bookmark, but the viewer is very unlikely to display
% anything beside the basic plane (unless one can change
% the UI's font).

% One could use a catcode table for this, but I don't think
% it's worth it.
{\catcode`\_=0
\catcode`\\=12
_gdef_navbackslash{\}}

\bgroup
\catcode`\%=12
\directlua{
local function to8 (...)
  local arg, str = {...}, ""
  for _, num in ipairs(arg) do
    str = str .. string.format("\noexpand\\navbackslash%.3o", num)
  end
  return str
end
function toutf16(str)
  local result = ""
  for c in string.utfvalues(str) do
    if c < 0x10000 then
      result = result .. to8(c / 256, c % 256)
    else
      c = c - 0x10000
      local a, b = c / 1024 + 0xD800, c % 1024 + 0xDC00
      result = result .. to8(a / 256, a % 256, b / 256, b % 256)
    end
  end
  tex.print([[\noexpand\navbackslash376\noexpand\navbackslash377]] .. result)
end
}
\egroup

\long\def\pdfstring#1{%
  \directlua{toutf16("\luaescapestring{#1}")}%
  }

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% Object creation %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\pdfobjectstatus#1{%
  \ifcs{nav@pdfobject:#1}
    {\ifcs{nav@pdfobject_used:#1}{2}{1}}
    {0}%
  }

\def\ifpdfobject#1{%
  \ifcs{nav@pdfobject:#1}%
  }

\def\pdfobject#1#2{%
  \nav@pdfobject{}{}[]{#1}{#2}%
  }

\def\pdfdictobject#1#2{%
  \nav@pdfobject{}{}[]{#1}{<< #2 >>}%
  }

\def\pdfstreamobject{%
  \ifnext[
    {\nav@pdfobject{stream}{}}
    {\nav@pdfobject{stream}{}[]}%
  }

\def\pdffileobject{%
  \ifnext[
    {\nav@pdfobject{stream}{file}}
    {\nav@pdfobject{stream}{file}[]}%
  }

\ifpdforluatex

\def\nav@pdfobject#1#2[#3]#4#5{%
  \ifnum\pdfobjectstatus{#4}=2
    \nav@error{There already exists an object named `#4'}%
  \else
    \immediate\pdfobj
    \ifnum\pdfobjectstatus{#4}=1 useobjnum \pdfobjectnumber{#4}\fi
    #1 % "stream" or nothing.
    \reverse\iffemptystring{#3}{attr {#3} }% "attr {...}" or nothing.
    #2 % "file" or nothing.
    {#5}% Contents.
    \ifnum\pdfobjectstatus{#2}=0
      \xdefcs{nav@pdfobject:#4}{\the\pdflastobj}%
    \fi
    \global\letcs{nav@pdfobject_used:#4}\relax
  \fi
  }

\def\pdfreserveobject#1{%
  \ifcase\pdfobjectstatus{#1}
    \pdfobj reserveobjnum
    \xdefcs{nav@pdfobject:#1}{\the\pdflastobj}%
  \or
    \nav@error{Object `#1' is already reserved}%
  \or
    \nav@error{Object `#1' is already in use}%
  \fi
  }

% An error message here wouldn't reach the terminal
% but would spoil the PDF file instead; therefore
% I prefer to return an unexisting (and impossible)
% object with number 0.

\def\pdfobjectnumber#1{%
  \ifcs{nav@pdfobject:#1}
    {\usecs{nav@pdfobject:#1}}
    {0}%
  }

\def\pdfrefobject#1{%
  \ifcs{nav@pdfobject:#1}
    {\usecs{nav@pdfobject:#1} 0 R}
    {0 0 R}%
  }

\else

\def\nav@pdfobject#1#2[#3]#4#5{%
  \ifnum\pdfobjectstatus{#4}=2
    \nav@error{There already exists an object named `#4'}%
  \else
    \special{pdf:
      \ifemptystring{#1}
        % No matter whether the object has been reserved,
        % it doesn't mean anything with xdvipdfmx.
        {obj \pdfrefobject{#4} #5}
        {\ifemptystring{#2}{stream}{fstream}
         \pdfrefobject{#4} (#5)
         \reverse\iffemptystring{#3}{<< #3 >>}}}%
    % Useless. But so the same behavior can be expected
    % no matter the driver.
    \global\defcs{nav@pdfobject:#4}{@nav_#4}%
    \global\letcs{nav@pdfobject_used:#4}\relax
  \fi
  }

\def\pdfreserveobject#1{%
  \ifcase\pdfobjectstatus{#1}
    % We do absolutely nothing except register the object
    % as ``reserved''.
    \xdefcs{nav@pdfobject:#1}{@nav_#1}%
  \or
    % Stupid, but then the same behavior can be expected
    % across engines.
    \nav@error{Object `#1' is already reserved}%
  \or
    \nav@error{Object `#1' is already in use}%
  \fi
  }

% We can't do anything meaningful here, so we do nothing.
\def\pdfobjectnumber#1{}

% With XeTeX, referencing of unreserved
% object is allowed, because reserving objects is
% dummy behavior anyway. Thus, rather than returning
% an unexisting 0 object, at least there exists the
% possibility that the object will be created later,
% even if it hasn't been reserved yet.
\def\pdfrefobject#1{@nav_#1}

\fi

\def\pdfensureobject#1{%
  \ifpdfobject{#1}{}{\pdfreserveobject{#1}}%
  }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% Anchors %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% REMARK
%
% Here and elsewhere, \usevalueor (or similar) is used (with a default
% value as the or-part), because the user might do something like:
%
% \setparameter param:
%   up = 12pt
%
% \anchor[meta = param]{foo}
%
% Then there is no value for the "left" attribute, since "param"
% doesn't have "navigator" (which holds the user's default values)
% as a meta-parameter.
% If no meta is detected, "navigator" is assigned to meta.

\def\nav@prepare_options#1#2{%
  \setparameterlist{nav@temp}[#1]{#2}%
  \nav@ifattribute nav@temp:meta;
    {}{\nav@setattribute nav@temp:meta; = navigator }%
  }

\def\anchor{%
  \ifnext[
    {\nav@anchor}
    {\nav@anchor[]}%
  }

\def\nav@anchor[#1]#2{%
  \ifcs{nav@pdfanchor:#2}
    {\nav@error{Anchor `#2' already exists}}
    {\global\letcs{nav@pdfanchor:#2}\relax
     \nav@prepare_options{\gobbleone}{#1}%
     \nav@anchor_position{#2}%
     \deleteparameter nav@temp:}%
  }

\def\nav@anchor_position#1{%
  \ifvmode
    \nav@passvalueand{\nav@anchor_pass{nav@pdfanchor:#1}}nav@temp:fit;{{\nav@usevalue nav@temp:zoom;}}
      {\nav@anchor_pass{nav@pdfanchor:#1}{xyz}{}}%
  \else
    \vbox to 0pt{\vss
      \vbox to \nav@usevalueor nav@temp:up;{\baselineskip}{%
        \hbox to 0pt{%
          \kern-\nav@usevalueor nav@temp:left;{0pt}%
          \nav@passvalueand{\nav@anchor_pass{nav@pdfanchor:#1}}nav@temp:fit;{{\nav@usevalue nav@temp:zoom;}}
            {\nav@anchor_pass{nav@pdfanchor:#1}{xyz}{}}\hss}\vss}}%
  \fi
  }

\def\nav@anchor_pass#1#2#3{%
  \lowercase{\nav@anchor_create{#2}}{#1}{#3}%
  }

\ifpdforluatex

\def\nav@anchor_xyz   #1{xyz zoom 0#1}
\def\nav@anchor_fit   #1{fit}
\def\nav@anchor_fith  #1{fith}
\def\nav@anchor_fitv  #1{fitv}
\def\nav@anchor_fitb  #1{fitb}
\def\nav@anchor_fitbh #1{fitbh}
\def\nav@anchor_fitbv #1{fitbv}
\def\nav@anchor_fitr  #1{fitr}

\def\nav@anchor_create#1#2#3{%
  \pdfdest name {#2} \ifcs{nav@anchor_#1}{\usecs{nav@anchor_#1}{#3}}{xyz}%
  }

\else

% FitR is quite unusable with xdvipdfm.
{\setcatcodes{pt=12}\gdef\noPT#1pt{#1}}
\def\nav@anchor_xyz   #1{XYZ   @xpos @ypos \expandafter\noPT\the\dimexpr0#1pt/1000\relax}
\def\nav@anchor_fit   #1{Fit}
\def\nav@anchor_fith  #1{FitH  @ypos}
\def\nav@anchor_fitv  #1{FitV  @xpos}
\def\nav@anchor_fitb  #1{FitB}
\def\nav@anchor_fitbh #1{FitBH @ypos}
\def\nav@anchor_fitbv #1{FitBV @xpos}

\def\nav@anchor_create#1#2#3{%
  \special{pdf: dest (#2)
    [ @thispage /\ifcs{nav@anchor_#1}{\usecs{nav@anchor_#1}{#3}}{XYZ} ]
    }%
  }

\fi

\def\anchorname#1{%
  nav@pdfanchor:#1%
  }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% Outlines %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\nav@pdfdef_list{}
\def\pdfdef#1{%
  \global\addright\nav@pdfdef_list{#1}%
  \gdefcs{nav@pdfdef:\commandtoname#1}%
  }

\newfor\nav@pdfdef_loop#1{%
  \lettocs#1{nav@pdfdef:\commandtoname#1}%
  }

\def\outline{%
  \ifnext[
    {\nav@outline}
    {\nav@outline[]}%
  }

\def\nav@outline[#1]#2{%
  \ifnext[
    {\nav@outline_do{#1}{#2}}
    {\nav@outline_do{#1}{#2}[]}%
  }

\newcount\nav@outline_count
\ifpdforluatex

\def\nav@outline_do#1#2[#3]#4{%
  \global\advance\nav@outline_count 1
  \gdefcs{nav@outline_\the\nav@outline_count:specs}{#1,}%
  \gdefcs{nav@outline_\the\nav@outline_count:level}{#2}%
  \gdefcs{nav@outline_\the\nav@outline_count:title}{#4}%
  \nav@prepare_options{\gobbleone}{#1}%
  \nav@outline_getaction{#1}{#3}%
  % It'd be simpler to create one action object anyway and let \nav@outline_n:action
  % refer to it; but then I'd have to use the /NoAction trick (in \nav@outline_getaction), which not all
  % viewers understand; at least here outlines with destinations work.
  \global\xdefcs{nav@outline_\the\nav@outline_count:action}{<< \nav@temp >>}%
  \deleteparameter nav@temp:%
  }

\def\nav@processoutlines{%
  \bgroup
  \passexpanded\nav@pdfdef_loop\nav@pdfdef_list
  \nav@processoutlines_loop{1}%
  \egroup
  }

\newwhile\nav@processoutlines_loop1{#1+1}
  {\straightenif{ifnum}{\numexpr#1>\nav@outline_count}
     {\breakwhile{}}
     {\nav@processoutlines_subloop{#1+1}{#1}{}{0}}%
  }

\newwhile\nav@processoutlines_subloop4{#1+1}{#2}{#3}{#4}
  {\straightenif{ifnum}{\numexpr#1>\nav@outline_count}
      {\breakwhile{\nav@processoutlines_create{#2}{#4}}}
      {\straightenif{ifdim}{\usecs{nav@outline_\the\numexpr#2:level}pt<\usecs{nav@outline_\the\numexpr#1:level}pt\relax}
         {\ifemptystring{#3}
            {\changewhile{#1+1}{#2}{#1}{#4+1}}
            {\reverse\straighteniff{ifdim}{\usecs{nav@outline_\the\numexpr#3:level}pt<\usecs{nav@outline_\the\numexpr#1:level}pt\relax}
               {\changewhile{#1+1}{#2}{#1}{#4+1}}}}
         {\breakwhile{\nav@processoutlines_create{#2}{#4}}}}%
  }

\def\nav@processoutlines_create#1#2{%
  \passexpandedcs{\nav@prepare_options{}}{nav@outline_\the\numexpr#1:specs}%
  \pdfoutline
    attr {\nav@outline_attributes}
    user {\usecs{nav@outline_\the\numexpr#1:action}}
    count \nav@ifvalue nav@temp:open; = true {}{-}\numexpr#2\relax {\pdfstring{\usecs{nav@outline_\the\numexpr#1:title}}}%
  \deleteparameter nav@temp:%
  }

\else
%
% So much simpler because xdvipdfmx deals with children
% automatically; thus \nav@processoutlines is unnecessary.
%

\let\nav@processoutlines\relax

\def\nav@outline_do#1#2[#3]#4{%
  \global\advance\nav@outline_count 1
  \nav@prepare_options{\gobbleone}{#1}%
  \nav@outline_getaction{#1}{#3}%
  \bgroup
  \passexpanded\nav@pdfdef_loop\nav@pdfdef_list
%  
  \special{pdf: out
    [\nav@ifvalue nav@temp:open;=true {}{-}] #2
    << /Title (#4)
       /A << \nav@temp >>
       \nav@outline_attributes >>}%
%
  \egroup
  \deleteparameter nav@temp:%
  }

\fi

\def\nav@outline_getaction#1#2{%
  \nav@storevalueand\nav@temp nav@temp:anchor;
    {\edef\nav@temp{/S/GoTo /D (\anchorname{\nav@temp})}}
    {\nav@storevalueand\nav@temp nav@temp:action;
      {\pdfensureobject{\nav@temp}%
       \edef\nav@temp{/S/Named /N/NoAction /Next \pdfrefobject{\nav@temp}}}
      {\nav@anchor[#1]{\ifemptystring{#2}{outline_\the\nav@outline_count}{#2}}%
       \edef\nav@temp{/S/GoTo /D (\anchorname{\ifemptystring{#2}{outline_\the\nav@outline_count}{#2})}}}}%
  }


\def\nav@outline_attributes{%
  % See REMARK above for default values.
  /C [\nav@usevalueor nav@temp:color;{\nav@usevalueor nav@temp:outlinecolor;{0 0 0}}]
  /F \nav@ifvalue nav@temp:bold; = true {1}{0}\nav@ifvalue nav@temp:italic; = true {1}{0}
  }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Annotations %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\actionlink{%
  \ifnext[
    {\nav@actionlink_do{a}}
    {\nav@actionlink_do{a}[]}%
  }

\def\rawactionlink{%
  \ifnext[
    {\nav@actionlink_do{r}}
    {\nav@actionlink_do{r}[]}%
  }

\def\jumplink{%
  \ifnext[
    {\nav@actionlink_do{d}}
    {\nav@actionlink_do{d}[]}% 
  }

\def\annotation{%
  \ifnext[
    {\nav@actionlink_do{x}}
    {\nav@actionlink_do{x}[]}% 
  }

\def\openfilelink{%
  \ifnext[
    {\nav@openfilelink}
    {\nav@openfilelink[]}%
  }

\def\nav@openfilelink[#1]#2{%
  \ifnext[
    {\nav@openfilelink_do{#1}{#2}}
    {\nav@openfilelink_do{#1}{#2}[0]}%
  }

\def\nav@openfilelink_do#1#2[#3]{%
  \nav@actionlink_do{r}[#1]
    {/S/GoToE /D [\the\numexpr#3-1\relax /Fit] 
     /T << /R/C /N (#2) >> /NewWindow true}%
  }

\long\def\nav@actionlink_do#1[#2]#3#4{%
  \nav@quitvmode
  \nav@prepare_options{}{#2}%
  \iffstring{#1}{a}{\pdfensureobject{#3}}%
  \nav@actionlink_create{#1}{#3}{%
    % Something in pre might be delimited by something in post
    % so post must be passed expanded.
    \nav@passvaluenobracesor{\nav@usevalue nav@temp:pre;#4}nav@temp:post;
      {\nav@usevalue nav@temp:pre;#4}%
    }%
  \deleteparameter nav@temp:%
  }

\ifpdforluatex

\let\nav@quitvmode\quitvmode

\long\def\nav@actionlink_create#1#2#3{%
  \pdfstartlink
  attr {\nav@actionlink_attributes{#1}{#2}}
  user {}%
  #3\pdfendlink
  }

\else

\let\nav@quitvmode\leavevmode

\long\def\nav@actionlink_create#1#2#3{%
  \special{pdf: bannot
    << \nav@actionlink_attributes{#1}{#2} >>}%
    #3\special{pdf: eannot}%
  }

\fi

\def\nav@actionlink_attributes#1#2{%
  /Border [0 0 \nav@usevalueor nav@temp:border;{1}%
      \nav@passvaluenobracesand{[}nav@temp:dash;{]}{}]
  /C [\nav@usevalueor nav@temp:color;{\nav@usevalueor nav@temp:linkcolor;{0 0 0}}]
  \nav@ifcasevalue nav@temp:highlight;%
  \val none    /H/N
  \val invert  /H/I
  \val outline /H/O
  \val push    /H/P
  \endval
  \ifstring{#1}{x}
    {#2}
    {/Subtype/Link
     \ifstring{#1}{d}
       {/Dest (\anchorname{#2})}
       {/A \ifstring{#1}{r}
           {<< #2 >>}
           {\pdfrefobject{#2}}}}%
  \nav@usevalue nav@temp:raw;%
  }

\pdfdictobject{firstpage}{/S/Named /N/FirstPage}
\pdfdictobject{lastpage} {/S/Named /N/LastPage}
\pdfdictobject{prevpage} {/S/Named /N/PrevPage}
\pdfdictobject{nextpage} {/S/Named /N/NextPage}

\def\urlaction#1#2{%
  \pdfdictobject{#1}{/S/URI /URI (#2)}%
  }

\def\javascriptaction#1#2{%
  \pdfdictobject{#1}{/S/JavaScript /JS (\pdfstring{#2})}%
  }

\def\urllink{%
  \ifnext[
    {\nav@urllink}
    {\nav@urllink[]}%
  }

\def\nav@urllink[#1]#2{%
  \nav@actionlink_do{r}[#1]{/S/URI /URI (#2)}%
  }

\def\javascriptlink{%
  \ifnext[
    {\nav@javascriptlink}
    {\nav@javascriptlink[]}%
  }

\def\nav@javascriptlink[#1]#2{%
  \nav@actionlink_do{r}[#1]{/S/JavaScript /JS (\pdfstring{#2})}%
  }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% Embedded files %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\nav@embeddedfile_names{}%

\ifcase\texenginenumber

\or % XeTeX
\def\nav@sort#1#2{%
  \straightenif{ifnum}{\strcmp{#1}{#2} < 0\relax}%
  }

\or % PDFTeX
\def\nav@sort#1#2{%
  \straightenif{ifnum}{\pdfstrcmp{#1}{#2} < 0\relax}%
  }

\or % LuaTeX
\def\nav@sort#1#2{%
  \usecs{%
    \directlua{%
      if [[#1]] < [[#2]] then
        tex.print("firstoftwo")
      else
        tex.print("secondoftwo")
      end}}}
\fi

\def\embeddedfile{%
  \ifnext[
    {\nav@embeddedfile_getdesc}
    {\nav@embeddedfile_getdesc[]}%
  }

\def\nav@embeddedfile_getdesc[#1]#2{%
  \ifnext[
    {\nav@embeddedfile_do{#1}{#2}}
    {\nav@embeddedfile_do{#1}{#2}[]}%
  }

\def\nav@embeddedfile_do#1#2[#3]#4{%s
  \pdffileobject[/Type/EmbeddedFile]{nav@embeddedfile:#2}{#4}%
  \pdfdictobject{#2}{%
    /Type/Filespec
    /F (\ifemptystring{#3}{#4}{#3})
    \reverse\iffemptystring{#1}{/Desc (\pdfstring{#1})}
    /EF << /F \pdfrefobject{nav@embeddedfile:#2} >>}%
  \let\nav@temp\nav@embeddedfile_names
  \let\nav@embeddedfile_names\emptycs
  \passexpanded{\ifemptystring{#3}{\nav@embeddedfile_add{#4}}{\nav@embeddedfile_add{#3}}{\pdfrefobject{#2}}}\nav@temp
  }

\newfor\nav@embeddedfile_add{2}#3#4{%
  \nav@sort{#1}{#3}
    {\global\eaddright\nav@embeddedfile_names{{#1}{#2}{#3}{#4}}%
     \retrieverest{\global\eaddright\nav@embeddedfile_names}}
    {\global\eaddright\nav@embeddedfile_names{{#3}{#4}}}%
  }[\global\eaddright\nav@embeddedfile_names{{#1}{#2}}]

\newfor\nav@embeddedfile_print#1#2{(#1) #2}

\def\nav@embeddedfile_process{%
  \pdfdictobject{EmbeddedFiles}{/Names [\passexpanded\nav@embeddedfile_print\nav@embeddedfile_names]}%
  \nav@embeddedfile_setnames
  }

\ifpdforluatex

\def\nav@embeddedfile_setnames{%
  \pdfnames{/EmbeddedFiles \pdfrefobject{EmbeddedFiles}}%
  }

\else

\def\nav@embeddedfile_setnames{%
  \special{pdf: put @names << /EmbeddedFiles \pdfrefobject{EmbeddedFiles} >>}%
  }

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% INFO %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifnav@finished
\def\finishpdffile{%
  \unless\ifnav@finished
    \global\nav@finishedtrue
    \nav@embeddedfile_process
    \nav@processoutlines
    \nav@processinfo
  \fi
  }

\setparameter navigator :
% ANCHORS (and bookmarks which create implicit anchors)
  up    = \baselineskip
  left  = 0pt
  fit   = xyz
%  zoom = 1000 % If it is set, it always sets view to 100%, which is extremely irritating.
%
% LINKS
  border    = 0
  linkcolor = "0 0 0" % "color" in individual links
  highlight = invert
% dash      = 1 0
% raw       = makes sense for individual links only
% pre       = nothing
% post      = nothing
%
% OUTLINES
  outlinecolor = "0 0 0" % "color" in individual outlines
  open         = false
  bold         = false
  italic       = false
% action       = makes sense for individual outlines only
% anchor       = idem
%
% PDF info, no default values:
% author, title, keywords, subject, date, moddate,
% creator, producer, rawinfo
%
% PDF catalog, idem:
% layout, mode, uri or base, openaction, rawcatalog


\def\nav@processinfo_do#1#2{%
  \nav@passvalueand{/#1 (\pdfstring}navigator:#2;{) }{}%
  }

\def\nav@processinfo{%
  \nav@info{%
    \nav@processinfo_do{Author}       {author}%
    \nav@processinfo_do{Title}        {title}%
    \nav@processinfo_do{Keywords}     {keywords}%
    \nav@processinfo_do{Subject}      {subject}%
    \nav@processinfo_do{CreationDate} {date}%
    \nav@processinfo_do{ModDate}      {moddate}%
    \nav@processinfo_do{Creator}      {creator}%
    \nav@processinfo_do{Producer}     {producer}%
    \nav@usevalue navigator:rawinfo;}%
%
  \nav@passvalue\pdfensureobject navigator:openaction;%
  \nav@catalog{%
    \nav@ifattribute navigator:layout;
      {/PageLayout%
       \nav@ifcasevalue navigator:layout;%
       \val onepage    /SinglePage
       \val onecolumn  /OneColumn
       \val twopage    /TwoPageRight
       \val twopage*   /TwoPageLeft
       \val twocolumn  /TwoColumnRight
       \val twocolumn* /TwoColumnLeft
       \endval\spacecs}{}%
    \nav@ifattribute navigator:mode;
      {/PageMode
       \nav@ifcasevalue navigator:mode;%
       \val outlines    /UseOutlines
       \val bookmarks   /UseOutlines
       \val thumbnails  /UseThumbs
       \val thumbs      /UseThumbs
       \val oc          /UseOC
       \val attachments /UseAttachments
       \val files       /UseAttachments
       \elseval         /UseOutlines
       \endval\spacecs}{}%
    \nav@ifattribute navigator:uri;
      {/URI << /Base (\nav@usevalue navigator:uri;) >> }
      {\nav@ifattribute navigator:base;
         {/URI << /Base (\nav@usevalue navigator:base;) >> }
         {}}%
    \nav@passvalue{/OpenAction \pdfrefobject}navigator:openaction;%
    \nav@usevalue navigator:rawcatalog;}%
  }%

\ifpdforluatex

\let\nav@info\pdfinfo
\let\nav@catalog\pdfcatalog

\else

\def\nav@info#1{%
  \special{pdf: docinfo << #1 >>}%
  }
\def\nav@catalog#1{%
  \special{pdf: docview << #1 >>}%
  }

\fi

\restorecatcodes
\endinput
% Almost 800 lines? Gee, that code was supposed to
% be short and light...

